A Unified Pilot Design for Integrated Sensing and Communications

This paper investigates a unified pilot signal design in an orthogonal frequency division modulation (OFDM)-based integrated sensing and communications (ISAC) system. The novel designed two-dimensional (2D) pilot signal is generated on the delay-Doppler (DD) plane for sensing, while its time-frequency (TF) plane transformation acts as the demodulation reference signal (DMRS) for the OFDM data. The well-designed pilot signal preserves orthogonality with the data in terms of resource occupancy in the TF plane and quasi-orthogonality in terms of codeword in the DD plane. Leveraging these nice properties, we are allowed to implement sensing detection in the DD plane using a simple 2D correlation, taking advantage of the favorable auto-correlation properties of the 2D pilot. In the communication part, the transformed pilot in the TF plane serves as a known DMRS for channel estimation and equalization. The 2D pilot design demonstrates good scalability and can adapt to different delay and Doppler resolution requirements without violating the OFDM data detection and can overcome the fractional Doppler with limited sensing resources. Experimental results show the effective sensing performance of the proposed pilot, with only a small fraction of power shared from the OFDM data,while maintaining satisfactory symbol detection performance in communication.

==> save.tex <==




\begin{align}
%\begin{split}
& v_{<l_0,k_0>} = <\mathbf{P}_{[l_0,k_0]},\mathbf{Y}\odot \Xi^{*}_{[l_0,k_0]}> \nonumber \\
& \approx \sum_{k=1}^{N}\sum_{l=1}^{M}p[[k-k_0]_N,[l-l_0]_M]*r_0[k,l] \nonumber \\
& *\alpha^{*}_{0}(k,l)e^{-j2\pi\frac{(L_{cp}+l-l_0)k_0}{N(M+L_{cp})}} \nonumber \\
& = h_0 \sum_{k=1}^{N}\sum_{l=1}^{M}h_0 p[[k-k_0]_N,[l-l_0]_M]*p[[k-k_0]_N,[l-l_0]_M] \nonumber \\
& + p[[k-k_0]_N,[l-l_0]_M]\alpha^{*}_{0}(k,l)\nonumber \\ 
& \left(\sum^{N_i}_{q=-N_i,q\neq 0}\alpha_{0}(k,l,q)p[[k-k_0+q]_N,[l-l_0]_M]e^{j2\pi\frac{(L_{cp}+l-l_0)\kappa_0}{N(M+L_{cp})}}\right) \nonumber \\
& = MNh_0 + h_0e^{j2\pi\frac{\kappa_0}{M+L_{cp}}}\nonumber \\
& \sum_{k=1}^{N}\sum_{l=1}^{M}e^{j2\pi\frac{(L_{cp}+l-l_0)}{N}}\alpha^{*}_{0}(k,l)p([k-k_0]_N,[l-l_0]_M) \nonumber \\
& \left(\sum_{q=-N_i,q\neq 0}^{N_i}{a_0(k,l,q)p([k-k_0+q]_N,[l-l_0]_M)}\right) \nonumber \\
& = MNh_0 + \mu(l_0,k_0,\kappa_0)h_0.
%\end{split}
\label{eq:eq17}
\end{align}

